Perceptual Artifacts Localization for Image Synthesis Tasks

Recent advancements in deep generative models have facilitated the creation of photo-realistic images across various tasks. However, these generated images often exhibit perceptual artifacts in specific regions, necessitating manual correction. In this study, we present a comprehensive empirical examination of Perceptual Artifacts Localization (PAL) spanning diverse image synthesis endeavors. We introduce a novel dataset comprising 10,168 generated images, each annotated with per-pixel perceptual artifact labels across ten synthesis tasks. A segmentation model, trained on our proposed dataset, effectively localizes artifacts across a range of tasks. Additionally, we illustrate its proficiency in adapting to previously unseen models using minimal training samples. We further propose an innovative zoom-in inpainting pipeline that seamlessly rectifies perceptual artifacts in the generated images. Through our experimental analyses, we elucidate several practical downstream applications, such as automated artifact rectification, non-referential image quality evaluation, and abnormal region detection in images. The dataset and code are released.

==> anyresgan.tex <==
\begin{figure}[!h]
\vspace{-10 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.05in 5.7in 8.9in 0in, clip,width=0.47\textwidth]{figs/anyresgan.pdf}
    \vspace{-10 pt}
    \caption{PAL and Artifacts Fixing for AnyRes GAN at resolution of 1024 $\times$ 1024. }
    \label{fig:anyresgan}
    \vspace{-10 pt}
\end{figure}






==> cross_domain_study.tex <==
\begin{table}[h!]
%   \vspace{-10 pt}
    \begin{center}
     \resizebox{0.48\textwidth}{!}{
      \begin{tabular}{l|c|c|c}
        \toprule % <-- Toprule here
        \textbf{Domains} \hspace{10pt} & \ \hspace{7pt} Face \hspace{7pt} & \ \hspace{7pt} Human \hspace{7pt} & \ \hspace{7pt} Animals \hspace{7pt}  \\
        \midrule
        Face & 41.65 & 23.94 & 12.14 \\
        Human & 16.71 & 37.57 & 9.17 \\
        Animal & 22.39 & 10.33 & 26.81 \\
        Joint Training & 42.16 & 36.72 & 25.58 \\
        \bottomrule
      \end{tabular}
      }
      \vspace{-5 pt}
      \caption{Cross-domain study in three domains using StyleGANs. Rows and columns indicate training and testing, respectively. The quantitative numbers indicate the mIoU. }
      \label{tab:cross_domain_study}
    \end{center}
    \vspace{-10 pt}
\end{table}





==> cross_model_study.tex <==
\begin{table}[h!]
    \begin{center}
     \resizebox{0.48\textwidth}{!}{
      \begin{tabular}{l|c|c}
        \toprule % <-- Toprule here
        \textbf{Models} \hspace{6pt} & \hspace{6pt} \ DALL-E 2 \hspace{6pt} & \ \hspace{6pt} Stable Diffusion \hspace{6pt}  \\
         \midrule
        DALL-E 2 & 26.47 & 24.59 \\
        Stable Diffusion & 20.27 & 24.27 \\
        Joint Training & 21.37 & 23.58 \\
        \bottomrule
      \end{tabular}
      }
      \vspace{-5 pt}
      \caption{Cross-model study on Text-to-Image synthesis task using DALL-E 2 and Stable Diffusion with COCO caption prompt. Rows and columns indicate training and testing, respectively. The quantitative numbers indicate the mIoU.}
      \label{tab:cross_model_study}
    \end{center}
    \vspace{-10 pt}
\end{table}




==> cross_resolution.tex <==
\begin{table}[h!]
    \begin{center}
     \resizebox{0.48\textwidth}{!}{
      \begin{tabular}{l|c|c|c}
        \toprule % <-- Toprule here
        \textbf{Resolutions} \hspace{0pt} & \hspace{0pt} \ 512 $\times$ 512 \hspace{0pt} & \hspace{0pt} \ 256 $\times$ 256  \hspace{0pt} & \hspace{0pt} \ 128 $\times$ 128  \hspace{0pt} \\
        \midrule % <-- Midrule here
        512 $\times$ 512 & 41.65 & 40.53 & 32.58 \\
        256 $\times$ 256 & 39.66 & 39.31 & 32.97 \\
        128 $\times$ 128 & 33.75 & 38.04 & 32.27 \\
        % Joint Training & - & - & - \\
        \bottomrule
      \end{tabular}
      }
      \vspace{-5 pt}
      \caption{Cross-resolution study on StyleGAN-FFHQ. Rows and columns indicate training and testing, respectively. The quantitative numbers indicate the mIoU.}
      \label{tab:cross_resolution_study}
    \end{center}
    \vspace{-10 pt}
\end{table}




==> cross_task_study.tex <==
\begin{table}[!h]
    \begin{center}
     \resizebox{0.48\textwidth}{!}{
      \begin{tabular}{l|c|c}
        \toprule % <-- Toprule here
        \textbf{Tasks} \hspace{6pt} & \hspace{3pt} \ Edge-to-Image \hspace{3pt} & \hspace{3pt} \ Mask-to-Image  \hspace{3pt} \\
        \midrule % <-- Midrule here
        Edge-to-Image & 45.56 & 39.62 \\
        Mask-to-Image & 44.63 & 35.01 \\
        Joint Training & 47.58 & 36.81 \\
        \bottomrule
      \end{tabular}
      }
      \vspace{-5 pt}
      \caption{Cross-task study on Edge-to-Image and Mask-to-Image. Rows and columns indicate training and testing, respectively. The quantitative numbers indicate the mIoU.}
      \label{tab:cross_task_study}
    \end{center}
    \vspace{-10 pt}
\end{table}




==> cvton.tex <==
\begin{figure}[!h]
\vspace{-12 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.0in 5.3in 8.5in 0in, clip,width=0.47\textwidth]{figs/cvton.pdf}
    \vspace{-10 pt}
    \caption{PAL and Artifacts Fixing for Virtual Try-On (VTON). }
    \label{fig:cvton}
    \vspace{-10 pt}
\end{figure}







==> edge2image.tex <==
\begin{figure}[!h]
\vspace{-14 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.05in 5.7in 8.9in 0in, clip,width=0.47\textwidth]{figs/edge2image.pdf}
    \vspace{-10 pt}
    \caption{PAL and Artifacts Fixing for Edge-to-Image translation. }
    \label{fig:edge2image}
    \vspace{-6 pt}
\end{figure}






==> generalization_analysis.tex <==
\begin{table*}[h!]
    \begin{minipage}[t]{0.4\textwidth}
     \centering
      \begin{tabular}
      {p{0.14\textwidth}p{0.12\textwidth}p{0.16\textwidth}p{0.17\textwidth}}
        \toprule % <-- Toprule here
        \textbf{Domains} & \ Face & \ Human & \ Animal  \\
        \midrule
        Face & - & - & - \\
        Human & - & - & - \\
        Animal & - & - & - \\
        Joint & - & - & - \\
        \bottomrule % <-- Bottomrule here
      \end{tabular}
      \caption{Cross-Domain study on StyleGANs. }
      \label{tab:cross_domain_study}
      \end{minipage}
      \begin{minipage}[t]{0.4\textwidth}
      \centering
      \begin{tabular}
      {p{0.17\textwidth}p{0.23\textwidth}p{0.17\textwidth}}
        \toprule % <-- Toprule here
        \textbf{Tasks} & \ StyleGAN & \ VTON  \\
         \midrule
        StyleGAN & - & - \\
        VTON & - & - \\
        Joint & - & - \\
        \bottomrule % <-- Bottomrule here
      \end{tabular}
      \caption{Cross-Task study on StyleGAN-Human and Virtual Try-On. }
      \label{tab:cross_task_study}
       \end{minipage}
      \begin{minipage}[t]{0.4\textwidth}
      \centering
      \begin{tabular}
      {p{0.33\textwidth}p{0.23\textwidth}p{0.34\textwidth}}
        \toprule % <-- Toprule here
        \textbf{Models} & \ DALL-E 2 & \ Stable Diffusion  \\
         \midrule
        DALL-E 2 & - & - \\
        Stable Diffusion & - & - \\
        Joint & - & - \\
        \bottomrule % <-- Bottomrule here
      \end{tabular}
      \caption{Cross-Model study on Text-to-Image Synthesis using DALL-E 2 and Stable Diffusion. }
      \label{tab:cross_task_study}
       \end{minipage}
\end{table*}







==> image_composition.tex <==
\begin{figure}[!h]
\vspace{-11 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.05in 5.7in 8.9in 0in, clip,width=0.47\textwidth]{figs/image_composition.pdf}
    \vspace{-10 pt}
    \caption{PAL and Artifacts Fixing for Image Composition.  }
    \label{fig:image_composition}
    \vspace{-10 pt}
\end{figure}






==> ldm.tex <==
\begin{figure}[!h]
 \vspace{-12 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.05in 5.7in 8.9in 0in, clip,width=0.47\textwidth]{figs/ldm.pdf}
    \vspace{-10 pt}
    \caption{PAL and Artifacts Fixing for a bedroom image generated by unconditional Latent Diffusion Models (LDMs). }
    \label{fig:ldm}
    \vspace{-10 pt}
\end{figure}






==> mask2image.tex <==
\begin{figure}[!h]
\vspace{-12 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.05in 5.7in 8.9in 0in, clip,width=0.47\textwidth]{figs/mask2image.pdf}
    \vspace{-10 pt}
    \caption{PAL and Artifacts Fixing for Mask-to-Image translation.  }
    \label{fig:mask2image}
    \vspace{-8 pt}
\end{figure}







==> psr.tex <==
\begin{figure}[!b]
\vspace{-15 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.0in 4.7in 8.6in 0in, clip,width=0.47\textwidth]{figs/psr.pdf}
    \vspace{-10 pt}
    \caption{PAL and Artifacts Fixing for Portrait Shadow Removal. }
    \label{fig:psr}
    % \vspace{-5 pt}
\end{figure}







==> rank_sd.tex <==
\begin{figure*}[!b]
 \vspace{-5 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0in 4.9in 1.1in 0in, clip,width=\textwidth]{figs/rank_sd.pdf}
    \vspace{-20 pt}
    \caption{Using Perceptual Artifacts Ratio as a metric to rank the multimodal outputs of text-to-image synthesis by Stable Diffusion. }
    \label{fig:rank_sd}
    \vspace{-10 pt}
\end{figure*}




==> stylegan2.tex <==
\begin{figure*}[!t]
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0in 4.1in 0.8in 0in, clip,width=\textwidth]{figs/stylegan2.pdf}
    \vspace{-20 pt}
    \caption{PAL and Artifacts Fixing for unconditional StyleGAN2 in domains: ffhq (left), afhqcat \& afhqdog (mild), StyleHuman (right). }
    \label{fig:stylegan2}
    \vspace{-15 pt}
\end{figure*}




==> super_resolution.tex <==
\begin{figure}[!h]
\vspace{-11 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.0in 5.7in 8.9in 0in, clip,width=0.47\textwidth]{figs/super_resolution.pdf}
    \vspace{-11 pt}
    \caption{PAL and Artifacts Fixing for super resolution using Real-ESRGAN, which upsamples an image by 4$\times$.  }
    \label{fig:super_resolution}
    \vspace{-10 pt}
\end{figure}




==> supp_zoom_inpaint_pipeline.tex <==
\begin{figure}[!h]
% \vspace{-5 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0in 1.8in 5.3in 0in, clip,width=0.47\textwidth]{figs/supp_zoom_inpaint_pipeline.pdf}
    % \vspace{-10 pt}
    \caption{A zoom-in inpainting pipeline that can fix perceptual artifacts for object details. In this pipeline, the original generated image is first cropped into multiple patches based on the perceptual artifacts segmentation. Afterwards, each cropped patch is fed into DALL-E 2 inpainting \cite{ramesh2022hierarchical} to fix the perceptual artifacts, and finally merged back into the full image. }
    \label{fig:supp_zoom_inpaint_pipeline}
    \vspace{-10 pt}
\end{figure}






==> text2image.tex <==
\begin{figure}[!h]
\vspace{-10 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.05in 5.3in 8.9in 0in, clip,width=0.47\textwidth]{figs/text2image.pdf}
    \vspace{-10 pt}
    \caption{PAL and Artifacts Fixing for Text-to-Image synthesis. }
    \label{fig:text2image}
    \vspace{-10 pt}
\end{figure}




==> zoom_in_comparison.tex <==
\begin{table}[!h]
    \begin{center}
     \resizebox{0.48\textwidth}{!}{
      \begin{tabular}{l|c|c|c}
        \toprule % <-- Toprule here
        \textbf{Methods} & \ Original & \ Naive Inpainting & \ Zoomed-in Inpainting  \\
        \midrule % <-- Midrule here
        PAR $\downarrow$ & - & - & - \\
        \midrule
        User Pref. $\uparrow$ & - & - & - \\
        \bottomrule
      \end{tabular}
      }
      \vspace{-5 pt}
      \caption{Quantitative evaluation of naive inpainting versus zoomed-in inpainting approaches. }
      \label{tab:zoom_in_comparison}
    \end{center}
    \vspace{-25 pt}
\end{table}

% Unified Model$^{*}$ indicates a unified model trained with balanced dataset.










==> zoom_in_fix.tex <==
\begin{figure}[!b]
\vspace{-5 pt}
    \centering
    %[trim=left bottom right top,
    \includegraphics[trim=0.0in 4.1in 4.2in 0in, clip,width=0.47\textwidth]{figs/zoom_in_fix.pdf}
    \vspace{-5 pt}
    \caption{... }
    \label{fig:zoom_in_fix}
    \vspace{-15 pt}
\end{figure}





